A Comprehensive Survey of Wireless Time-Sensitive Networking (TSN): Architecture, Technologies, Applications, and Open Issues

Time-sensitive networking (TSN) is expected to be a key component of critical machine-type communication networks in areas such as Industry 4.0, robotics and autonomous vehicles. With rising mobility requirements in industrial applications and the prevalence of wireless networks, wireless network integration into TSN is becoming increasingly important. This survey article presents a comprehensive review of the current literature on wireless TSN, including an overview of the architecture of a wireless TSN network and an examination of the various wireless technologies and protocols that can be or are used in such networks. In addition, the article discusses industrial applications of wireless TSN, among them industrial automation, robotics, and autonomous vehicles. The article concludes by summarizing the challenges and open issues related to the integration of TSN into wireless networks, and by offering suggestions for future research directions.

==> Authors-bio-photos/Authors-Bio.tex <==

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.75in, clip, keepaspectratio]{Authors-bio-photos/Kouros.jpg}}]{Kouros Zanbouri} received a BSc degree in Information Technology (IT) engineering in 2016 and pursued an MSc degree in IT engineering - specializing in Computer Networks, in 2018. Kouros is currently conducting research on Time-Sensitive Networking (TSN) as a Ph.D. Student at UCC, in CONNECT Centre, School of Computer Science \& IT, University College Cork, Ireland.
\end{IEEEbiography}
\vskip 0pt plus -1fil % Reduce space between biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.75in,clip,keepaspectratio]{Authors-bio-photos/DrRahim2.jpg}}]{Md. Noor-A-Rahim} received the Ph.D. degree from the School of Information Technology and Mathematical Sciences, University of South Australia, Australia in 2015. Dr. Rahim is currently serving as an Assistant Professor (Lecturer-Above the Bar) within the School of Computer Science and Information Technology at University College Cork, Ireland. Prior to this role, he was a Senior Researcher and Marie Curie Fellow within the same school. He also held the position of Postdoctoral Research Fellow at the Nanyang Technological University (NTU), Singapore. His research interests include Control over Wireless Networks, Intelligent Transportation Systems,  Machine Learning, Signal Processing, and DNA-based Data Storage. In recognition of his academic excellence, he was honored with the Michael Miller Medal for presenting the most outstanding Ph.D. thesis in 2015. For more details, please visit: https://narahim.github.io/
\end{IEEEbiography}
\vskip 0pt plus -1fil % Reduce space between biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.75in, clip, keepaspectratio]{Authors-bio-photos/Jobish_John.jpg}}]{Jobish John} received Ph.D. in Electrical Engineering from Indian Institute of
Technology, Bombay in 2020. He is currently working as a post-doctoral researcher at The Centre for Wireless Technology Eindhoven (CWTe), Department of Electrical Engineering, Eindhoven University of technology, The Netherlands. Before this role, he was a Marie Curie Fellow with the School of Computer Science and Information Technology, University College Cork, Ireland. His main research interests lie in the area of next-generation wireless networks. This ranges from ultra reliable and low latency communication systems for various verticals such as avionics, Industry 4.0/5.0, to Internet of Things and Low -Power Wide Area Networks. to distributed, heterogeneous, self-organizing networks.
\end{IEEEbiography}
\vskip 0pt plus -1fil % Reduce space between biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.75in, clip, keepaspectratio]{Authors-bio-photos/Cormac.JPG}}]{Cormac J. Sreenan} is Professor of Computer Science at University College Cork in Ireland where he leads a research team working on wireless and mobile networking, funded by Science Foundation Ireland, the EU, Enterprise Ireland, and numerous companies. Prior to joining UCC he was a research scientist at AT\&T (Bell) Labs in NJ USA. He has a Ph.D. from the University of Cambridge, and is a Fellow of the Irish Academy of Engineering, a Life Fellow of the Cambridge Philosophical Society, and a Senior Member of the IEEE.
\end{IEEEbiography}
\vskip 0pt plus -1fil % Reduce space between biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.75in,clip,keepaspectratio]{Authors-bio-photos/poor-v.jpg}}]{H. Vincent Poor} (S’72, M’77, SM’82, F’87) received the Ph.D. degree in EECS from Princeton University in 1977.  From 1977 until 1990, he was on the faculty of the University of Illinois at Urbana-Champaign. Since 1990 he has been on the faculty at Princeton, where he is currently the Michael Henry Strater University Professor. During 2006 to 2016, he served as the dean of Princeton’s School of Engineering and Applied Science, and he has also held visiting appointments at several other universities, including most recently at Berkeley and Caltech. His research interests are in the areas of information theory, machine learning and network science, and their applications in wireless networks, energy systems and related fields. Among his publications in these areas is the book Machine Learning and Wireless Communications. (Cambridge University Press, 2022). Dr. Poor is a member of the National Academy of Engineering and the National Academy of Sciences and is a foreign member of the Royal Society and other national and international academies. He received the IEEE Alexander Graham Bell Medal in 2017.
\end{IEEEbiography}
\vskip 0pt plus -1fil % Reduce space between biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.75in, clip, keepaspectratio]{Authors-bio-photos/Dirk.jpg}}]{Dirk Pesch}(Senior Member, IEEE) received the Dipl.Ing. degree from RWTH Aachen University, Aachen, Germany, and the Ph.D. degree from the University of Strathclyde, Glasgow, U.K. He is currently a Professor and Head of School of the School of Computer Science and Information Technology at University College Cork, Ireland. Dirk has more than 25 years research and development experience in both industry and academia and has authored or coauthored more than 200 scientific articles and book chapters. His research interests include architecture, design, algorithms, and performance evaluation of low power, dense and mobile wireless networks and services for Internet of Things and Cyber-Physical System's applications in smart connected communities, health and wellbeing, and smart manufacturing. He is a Principal Investigator of the Science Foundation Ireland funded CONNECT Centre for Future Networks and the Director of the SFI Centre for Research Training in Advanced Networks for Sustainable Societies. Dirk contributes to international conference organization and is a Member of the Editorial Board of a number of journals.
\end{IEEEbiography}
